A Prosumer-Centric Framework for Concurrent Generation and Transmission Planning -- Part I

The growing share of proactive actors in the electricity markets calls for more attention on prosumers and more support for their decision-making under decentralized electricity markets. In view of the changing paradigm, it is crucial to study the long-term planning under the decentralized and prosumer-centric markets to unravel the effects of such markets on the planning decisions. In the first part of the two-part paper, we propose a prosumer-centric framework for concurrent generation and transmission planning. Here, three planning models are presented where a peer-to-peer market with product differentiation, a pool market and a mixed bilateral/pool market and their associated trading costs are explicitly modeled, respectively. To fully reveal the individual costs and benefits, we start by formulating the optimization problems of various actors, i.e. prosumers, transmission system operator, energy market operator and carbon market operator. Moreover, to enable decentralized planning where the privacy of the prosumers is preserved, distributed optimization algorithms are presented based on the corresponding centralized optimization problems.

==> nomenclature.tex <==
\section*{Nomenclature}
% \addcontentsline{toc}{section}{Nomenclature}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$PTDF$}]

\item[\textbf{Sets}]
\item[$\mathcal{G}$] Set of generation technologies
\item[$\mathcal{L}$] Set of lines
\item[$\mathcal{N}$] Set of prosumers/line nodes
\item[$\mathcal{R}$] Set of fossil-fueled generation
\item[$\mathcal{S}$] Set of storage technologies
\item[$\mathcal{T}$] Set of time steps
\item[$\omega_n$] Set of neighbors of prosumer $n$ on the communication graph 
\item[$\Gamma$] Set of decision variables 

\item[\textbf{Parameters}]
\item[$A_{i}$] Annuity factor of technology $i$
\item[$A_l$]  Annuity factor of line $l$
\item[$B_{i}$] Variable Operation \& Maintenance costs (VOM)  of technology $i$
\item[$C_{i}$] Capital Expenditures (CapEx) and Fixed Operation \& Maintenance costs (FOM) of generation technology $i$
\item[$CS_{i}$] Capital Expenditures (CapEx) and Fixed Operation \& Maintenance costs (FOM) of storage technology $i$ 
\item[$C_l$] Capital Expenditures (CapEx) and Fixed Operation \& Maintenance costs (FOM) of line $l$
\item[$E_i$] emission of fossil-fueled technology $i$ 
\item[$H^{in}_{i}$] Charging efficiency of storage technology $i$
\item[$H^{out}_{i}$] Discharging efficiency of storage technology $i$
\item[$I_{n,m}$] Preference value from prosumer $n$ towards prosumer $m$
\item[$K_{i,n}$] Existing capacity of technology $i$ for prosumer $n$
\item[$K_l$] Existing capacity of line $l$

\item[$\Delta_l$] length of line $l$
\item[$PTDF$] Power Transfer Distribution Factors (PTDF) matrix
\item[$\Phi_n$] Percentage of trades in the bilateral market for prosumer $n$

\item[\textbf{Variables}]
\item[$f_{l,t}$] Energy flow at line $l$ at time step $t$
\item[$f_n$] Summation of CapEx, FOM, VOM for prosumer $n$
\item[$k_{i,n}$] Investment capacity of generation technology $i$ for prosumer $n$
\item[$k^{\text{storage}}_{i,n}$] Investment capacity of storage technology $i$ for prosumer $n$
\item[$k_l$] Investment capacity of line $l$
\item[$p_{i,n,t}$] Produced energy from technology $i$ from prosumer $n$ at time step $t$
\item[$p^{\text{trade}}_{n,m,t}$] Trade energy from prosumer $n$ to prosumer $m$ at time step $t$
\item[$p^{\text{in}}_{i,n,t}$] Charging to storage of storage technology $i$ for prosumer $n$ at time step $t$
\item[$p^{\text{out}}_{i,n,t}$] Discharging from storage of storage technology $i$ for prosumer $n$ at time step $t$
\item[$soc_{i,n,t}$] Energy in storage of storage technology $i$ for prosumer $n$ at time step $t$
\item[$z^{\text{net}}_{n,m,t}$] Arbitrage energy from the Transmission System Operator (TSO) from node $n$ to node $m$ at time step $t$
\item[$z^{\text{net}}_{n,t}$] Arbitrage energy from the TSO at node $n$ at time step $t$
\item[$\lambda^{\text{trade}}_{n,m,t}$] Trade price between prosumer $n$ and prosumer $m$ at time step $t$
\item[$\lambda^{\text{grid}}_{n,m,t}$] Grid price between prosumer $n$ and prosumer $m$ at time step $t$
\item[$\lambda_{n,t}$] Nodal price at node $n$ at time step $t$
\item[$g$] CapEx for TSO





\end{IEEEdescription}

